A Tale of Two Classes: Adapting Supervised Contrastive Learning to Binary Imbalanced Datasets

Supervised contrastive learning (SupCon) has proven to be a powerful alternative to the standard cross-entropy loss for classification of multi-class balanced datasets. However, it struggles to learn well-conditioned representations of datasets with long-tailed class distributions. This problem is potentially exacerbated for binary imbalanced distributions, which are commonly encountered during many real-world problems such as medical diagnosis. In experiments on seven binary datasets of natural and medical images, we show that the performance of SupCon decreases with increasing class imbalance. To substantiate these findings, we introduce two novel metrics that evaluate the quality of the learned representation space. By measuring the class distribution in local neighborhoods, we are able to uncover structural deficiencies of the representation space that classical metrics cannot detect. Informed by these insights, we propose two new supervised contrastive learning strategies tailored to binary imbalanced datasets that improve the structure of the representation space and increase downstream classification accuracy over standard SupCon by up to 35%. We make our code available.

==> sec/1_intro_old.tex <==
\section{Introduction and Related Work}
\label{sec:intro}

\begin{figure}[tb]
  \centering
  \includegraphics[width=1.0\linewidth]{figures/1/Figure1BinCL.drawio.pdf}
  \caption{Supervised contrastive learning works well on multi-class datasets but fails to train on imbalanced binary datasets, collapsing to a single embedding. Our methods prevent this collapse allowing for a clear separation of the classes and strong downstream classification performance.}
  \label{fig:graphical_abstract}
\end{figure}

%todo find a source that supervised cl is still hot topic in 2024 sota for supervised representation learning experiences revival with transformer architectures:

Supervised contrastive learning (SupCon) has emerged as a powerful alternative to the cross-entropy loss for learning high-quality representations using full label information \cite{DBLP:journals/corr/abs-2004-11362,graf2023dissecting,li2022targeted,li2022selective}.
However, SupCon has been predominantly developed and applied on balanced multi-class benchmark datasets like ImageNet, which consist of many evenly distributed classes. On such distributions, SupCon learns a well-conditioned representation space, which preserves discriminative features of each sample while separating semantic classes~\cite{assran2022hiddenuniformclusterprior}. 

In contrast, real-world datasets often significantly deviate from these idealized conditions. Particularly in medical imaging applications, datasets frequently contain binary and heavily imbalanced semantic classes~\cite{healthcare10071293,Hee_2022}. For example, during clinical diagnosis or screening, subjects are classified as either healthy or diseased, with the healthy cases significantly outnumbering the pathological ones. A survey on transfer learning for medical image classification found that 78 out of 114 studies focused on binary classification problems~\cite{Hee_2022}. 
%long tail benchmark datasets also do not capture distribution of medical problems: data collected from hospitals is often labeled solely for the purpose of the study, and the prevalence of certain diseases leads to inherent class imbalances. 
% Given that features often do not transfer effectively across different domains~\cite{DBLP:journals/corr/abs-2105-05837}, learning a well-conditioned representation space directly from binary, imbalanced data distributions is essential in medical contexts.

%supcon sota but doesnt work for this important distribution as we show:

In this work we empirically demonstrate and theoretically substantiate that SupCon has greatly diminished effectiveness on binary imbalanced distributions. 
Specifically, it fails to learn an expressive representation space because it concentrates representations too close together which can lead to representation collapse at higher data imbalances (see \cref{fig:graphical_abstract}).
While existing literature has diagnosed and improved the performance of SupCon on multi-class long-tailed distributions \cite{zhu2022balanced,hou2023subclass,DBLP:journals/corr/abs-2107-12028,kang2021exploring,li2022targeted}, many of these methods struggle on binary imbalanced datasets.

%In heavily imbalanced datasets, training batches are dominated by samples from the majority class, leading to negatives that predominantly share the same semantic features. This scenario causes the model to overlook shared features within the majority class, impeding the development of a discriminative feature space. As a result, the quality and utility of the learned representations for downstream tasks are significantly compromised.
% Potentially remove: Beyond their practical utility, binary contrastive learning provides a unique lens for analyzing representation spaces. Any dataset can be artificially converted into a binary classification problem through one-vs-all label aggregation into super-classes or by considering the presence or absence of a specific feature. 
% By examining how well binary features or super-classes are learned, we gain insight into how contrastive learning captures desired features. These findings can inform strategies for improving representation quality and managing class imbalances in larger, multi-class datasets.
%we try to identify the problems by extending established representation space metrics for unsupervised cl to the supervised case and analyse representation space on artificially datasets for which we control class imbalances:
To evaluate the quality of obtained representation spaces and the effect under varying number of semantic classes and label imbalance, others have introduced the notion of representation space alignment and uniformity \cite{DBLP:journals/corr/abs-2005-10242}. Alignment measures similarity between data representations and uniformity measures representation spread across the latent space. However, these definitions do not take into account the relationship \textit{between} embeddings of different classes, which is the deciding factor for downstream classification performance. We fill this gap by introducing novel metrics, enabling the evaluation of class consistency within representation neighborhoods. %Additionally, we propose a probabilistic definition of uniformity that relaxes the requirement of local representation uniformity.

%substantiate our empirical findings by mathematical formalization / proof


Building on insights gained from our novel metrics, we propose targeted adjustments to SupCon that enhance class alignment while facilitating the formation of an expressive feature space. These adjustments are easy to implement and have minimal additional computational cost. Through extensive experiments on both natural image and medical datasets, we demonstrate that our proposed methods improve accuracy by up to 35\% over standard cross entropy and supervised contrastive learning and outperform leading methods in the literature by up to 10\%.

%In conclusion, our novel metrics more effectively predict downstream utility than canonical metrics and have guided the development of modifications to supervised contrastive learning that excel on both balanced and imbalanced binary data. By focusing on the unique challenges of imbalanced binary datasets, we advance tools and methods to better handle these common real-world data distributions, particularly in medical applications.




%In summary, we make the following contributions:

%\begin{itemize} 
%\item We empirically and mathematically demonstrate the diminished effectiveness of supervised contrastive learning on imbalanced binary datasets, often resulting in complete representation collapse. 
%\item We introduce novel metrics to assess the structure and quality of the representation spaces obtained. Specifically, we extend the concept of alignment to latent class labels, enabling the evaluation of class consistency within representation neighborhoods. Additionally, we propose a probabilistic definition of uniformity that relaxes the requirement of local representation uniformity. 
%\item Finally, we propose two new supervised contrastive learning strategies for imbalanced binary datasets. Our methods, informed by the insights gained through our metrics, improve both alignment and uniformity, leading to enhanced downstream classification performance on both natural image and medical datasets. 
%\end{itemize}

==> sec/2_related_work_old.tex <==
\section{Related work}
\label{sec:related_work}

\paragraph{Supervised contrastive learning}

SupCon has emerged as an effective improvement upon the conventional cross-entropy loss \cite{DBLP:journals/corr/abs-2004-11362}. SupCon effectively extends the cross-entropy loss from a single class label to include all representations from the same class. This provides a strong signal to align the representations of a class, while still contrasting against samples from other classes to prevent a degenerate solution. Since the representations are also normalized onto a unit hypersphere, SupCon simultaneously spreads representations while actively aligning the latent classes, thus ensuring the learned representations are both generalizable and separable. 

\paragraph{Supervised contrastive learning for long-tailed datasets}

While SupCon works well on balanced datasets, on long-tailed datasets the representation space typically becomes biased towards the majority class \cite{zhu2022balanced, li2022targeted, DBLP:journals/corr/abs-2107-12028,kang2021exploring, hou2023subclass}. In the most severe cases the representations collapse completely, losing all utility \cite{pmlr-v202-xue23d,Hager_2023_CVPR,chen2022perfectly,graf2023dissecting}.

%Originally, multi-class long-tailed distributions often relied on bias reduction techniques such as data resampling \cite{ando2017deep,buda2018systematic} and loss reweighting \cite{byrd2019effect,cao2019learning}. However, deploying these methods in binary classification scenarios, especially with highly imbalanced datasets, is ineffective. For a 1\% imbalance, resampling would entail either discarding up to 99\% of the training batch or substantial data duplication, reducing the information content of gradient updates. Similarly, adjusting the loss function to counteract such extreme imbalance would result in the minority class contributing disproportionately more to the loss than the majority class, potentially by a factor of up to 99.

Many works thus aim to enhance latent space uniformity, spreading features evenly, irrespective of data imbalance. Zhu \etal balance gradient contributions of classes to achieve a regular simplex latent structure \cite{zhu2022balanced}. Hou \etal split the majority classes into smaller sub-classes according to their latent features \cite{hou2023subclass}.
Cui \etal leverage parametric class prototypes to adaptively balance the learning signal \cite{DBLP:journals/corr/abs-2107-12028}. Kang \etal and Li \etal limit the number of positives that contribute to the loss with Li \etal also using fixed class prototypes \cite{kang2021exploring, li2022targeted}. 
While these methods have been shown to surpass SupCon on long-tailed distributions, the unique characteristics of binary distributions require tailored solutions. 
% allow us to simplify and improve upon them, to reduce both complexity and overhead while increasing performance.
%Although these methods increase the alignment of the learned representations and class uniformity, they reduce sample uniformity resulting in diminished downstream utility.

\paragraph{Analyzing contrastive representation spaces}

To analyze latent spaces and the functioning of supervised contrastive learning methods on binary, imbalanced datasets, we build upon previous research that has investigated the links between contrastive learning training dynamics, the obtained representation space, and ultimate downstream performance. 
%Arora \etal and Lee  \etal\cite{DBLP:journals/corr/abs-1902-09229, DBLP:journals/corr/abs-2008-01064} introduced the concepts of semantic similarity and latent classes, positing that similar pairs are assumed to be drawn from the same latent class and that a downstream task is comprised of a subset of these latent classes. 
%Their work also discusses false negatives, referred to as class collisions, and their detrimental effects on representation quality. 
%These insights support and motivate our hypothesis that imbalanced binary datasets lead to misalignment in learned similarity because negatives are mostly drawn from the same latent class.
Wang and Isola \cite{DBLP:journals/corr/abs-2005-10242} have shown that contrastive learning optimizes for alignment and uniformity. These characteristics have been empirically validated as strong indicators of the representation space's quality and downstream utility. However, high uniformity and alignment alone do not guarantee separated latent classes, as shown by Wang \etal \cite{wang2022chaos}. 
To better understand the connection between the representation space and the downstream classification performance, Li \etal suggested analyzing alignment and uniformity on the level of class, and not just instance \cite{li2022targeted}.
While this is an improvement over sample-wise analysis, it still fails to properly compare representations \textit{between} classes, which ultimately decides downstream performance.
% We expand upon these concepts and adapt them to the binary case, suggesting additional metrics that examine class neighborhoods to better illuminate the trained representation spaces.


% \paragraph{Unsupervised long-tail contrastive learning}

% Most efforts to improve unsupervised long-tail contrastive learning aim to identify tail samples and adjust their bias relative to head samples. Proposed solutions include the analysis of memorization in the encoder network \cite{jiang2021selfdamaging,zhou2022contrastive}, or interpreting the obtained representation space using clustering, support views, or training prototypes \cite{DBLP:journals/corr/abs-2106-03719, Tejankar_2021_ICCV, DBLP:journals/corr/abs-2011-11765,lin2023frequencyaware}. Others have attempted to define a distribution over hard negative pairs, but the success of this approach hinges on the data matching the assumed distribution \cite{robinson2021contrastive}. However, all of the proposed strategies are inherently unsuitable for the binary scenario, as the ability to successfully distinguish head from tail samples presupposes the completion of the downstream classification task.

